Is SP BP?

The Survey Propagation (SP) algorithm for solving $k$-SAT problems has been shown recently as an instance of the Belief Propagation (BP) algorithm. In this paper, we show that for general constraint-satisfaction problems, SP may not be reducible from BP. We also establish the conditions under which such a reduction is possible. Along our development, we present a unification of the existing SP algorithms in terms of a probabilistically interpretable iterative procedure -- weighted Probabilistic Token Passing.

==> bp.tex <==
\section{The Reduction of SP from BP}
\label{sec:bp}

\subsection{The reduction of SP from BP for arbitrary CSP}
\subsubsection{Extended symbol variables and state variables}
Given a CSP  represented by factor graph $G$, for each variable
$x_v$, we introduce an extended symbol variable (referred to as
symbol variable hereafter) $y_v$, taking values from the extended
alphabet $\chi_v^*$.

For each edge $(x_v,\Gamma_c)\in E(G)$, we introduce a generalized
state variable (referred to as state variable hereafter) $s_{v,c}$
which takes on values in set $\chi_v^*\times\chi_v^*$. Each state
variable $s_{v,c}$ will also be written as an ordered pair
$(s_{v,c}^L,s_{v,c}^R)$, where the first component is referred to as
the left state, and the second component is referred to as the right
state. For any $v\in V$ and any subset $C'\subseteq C(v)$, we use
$s_{v,C'}$ to denote the variable set $\{s_{v,c}:c\in C'\}$.
Likewise, for any $c\in C$ and any subset $V'\subseteq V(c)$, we use
$s_{V',c}$ to denote the variable set $\{s_{v,c}:v\in V'\}$. In
addition, we will use $s_{V,C}$ to denote the set of all state
variables. Similar notations apply to left and right states.

\subsubsection{Normal realizations}
We will now introduce a MRF defined on $\chi_V^*$. The local
potential functions of the MRF consist of {\em left functions} ---
each for a $v\in V$ and denoted by $g_v$ --- and a set of {\em right
functions} --- each for a $c\in C$ and denoted by $f_c$. The left
function $g_v$ for each $v\in V$ is defined as

\begin{equation}
\label{equ:leftfunction}
g_v(y_v,s_{v,C(v)}):=W_L(y_v,s_{v,C(v)})\cdot[y_v\subseteq\bigcap_{c\in
C(v)}s^R_{v,c}]\cdot\prod_{c\in
C(v)}[s^L_{v,c}=
%\left(\bigcap_{c'\in
%C(v)\setminus\{c\}}s^R_{v,c'}\right)\cap 
y_v]
\end{equation}
where $W_L(y_v,s_{v,C(v)})$ is a non-negative weighting function.

{\bf [check with ITW paper to verify the above equation -- checked! Fine.
]}

The right function $f_c$ for each $c\in C$ is defined as

\begin{equation}
\label{equ:rightfunction}
f_c(s_{V(c),c}):=W_R(s_{V(c),c})\cdot\prod_{v\in
V(c)}[s^R_{v,c}={\tt F}_c(s^L_{V(c)\setminus\{v\},c})]
\end{equation}
where $W_R(s_{V(c),c})$ is another non-negative function.

We then define a global function $F$ via the above-defined local
functions:

\begin{equation}
\label{equ:globalfunction} F(y_V,S{V,C}):=\prod_{v\in
V}g_v(y_v,s_{v,C(v)})\cdot\prod_{c\in C}f_c(s_{V(c),c}).
\end{equation}

Then function $F$ is readily expressed as a factor graph. Notice
that in this factor graph, all symbol variables have degree one and
all state variables have degree two, giving rise to a normal
realization \cite{Forney:normalGraph}. Following
\cite{Forney:normalGraph}, such a factor graph can be more compactly
represented as a Forney graph, where each state variable is
represented as an edge, each side variable represented as a terminal
or ``half-edge'', and local functions represented as nodes. The
Forney graph representing the normal realization of the toy 3-SAT
problem in Figure  \ref{fig:ksat_fg} is shown in Figure
\ref{fig:ksat_forneyG}.

\begin{figure}[htb]
\begin{center}
  \scalebox{0.45}{\input{fig/fig2.pstex_t}}
  \caption{The Forney graph representing the normal realization of the
toy problem in Figure \ref{fig:ksat_fg}.}
  \label{fig:ksat_forneyG}
\end{center}
\end{figure}

As is standard, when treating function $F$ (upon normalization) as a
probability mass function, the factorization structure of $F$
defines an MRF.

\begin{lem}
If the weighting functions $W_L(\cdot)$ and $W_R(\cdot)$ are
strictly positive, then for every sequence $(y_V,s_{V,C})$ in the
support of $F$, it holds that
\[
s_{v,c}^L\subseteq y_v\subseteq s_{v,c}^R
\]
for every $(v,c)$ such that $(x_v,\Gamma_c)\in E(G)$.
\end{lem}

{\bf  The result in the above lemma is not accurate, or quite loose. 
In fact, I believe the correct one should be
\[
s_{v,c}^L =  y_v\subseteq s_{v,c}^R
\]
which directly follows from the definition of the left function. -- This lemma 
may be removed, to be decided after checking out how it is used later.
}

\begin{proof}
This lemma can be proved directly from the definition of local
function $g_{v}(y_v,s_{v,C(v)})$ .
\end{proof}

\subsubsection{State-decoupled BP}
We now introduce a message-passing rule on the Forney graph, which
we refer to as the {\em state-decoupled belief propagation} (SD-BP).
The purpose of introducing this ``new'' message-passing rule is to
arrive at a unified reduction mechanism for SP to reduce from BP (or
more precisely from SD-BP).

Identical to BP at local function vertices, SD-BP differs from BP in
that messages passed from the right functions need an additional
processing, which we call {\em state decoupling}, before they are
passed to the left functions. More precisely, there are three kinds
of messages: {\em right message} $\rho_{c\rightarrow v}$ is computed
at right function $f_c$ to pass along the edge to $g_v$;
state-decoupled right message $\rho_{c\rightarrow v}^*$ is computed
at the edge connecting $f_c$ and $g_v$, which depends only on the
right message $\rho_{c\rightarrow v}$ on the same edge and is passed
to left function $g_v$; {\em left message} $\lambda_{v\rightarrow
c}$ is computed at the left function $g_v$ to pass along the edge
connecting to $f_c$. We note that the state-decoupled right message
$\rho^*_{c\rightarrow v}$ is a function on support of
$\rho_{c\rightarrow v}$ satisfying the following property:
$\rho^*_{c\rightarrow v}(s^L_{v,c},s^R_{v,c})=\rho^*_{c\rightarrow
v}(s^R_{v,c},s^R_{v,c})$ for every $s^L_{v,c}\in \chi_v^*$ and
$s^R_{v,c}\in \chi^*_v$ such that $(s^L_{v,c},s^R_{v,c})$ and
$(s^R_{v,c},s^R_{v,c})$ are in the support of $\rho_{c\rightarrow
v}$. An intuitive explanation of state decoupling is to result in
that the (state-decoupled) right messages only depend on their right
states. We define the state-decoupling operation as follows:
$\rho^*_{c\rightarrow v}(s^L_{v,c},s^R_{v,c}):=\rho_{c\rightarrow
v}(s^R_{v,c},s^R_{v,c})$ for every $(s^L_{v,c},s^R_{v,c})$ in the
support of $\rho_{c\rightarrow v}$.

More precisely, the SD-BP message passing rule is given as follows.
\begin{equation}
\label{equ:sd_bp_leftmessage} \lambda_{v\rightarrow
c}(s^L_{v,c},s^R_{v,c})=\sum_{{s^R_{v,C(v)\setminus\{c\}}:}\atop{s^L_{v,c}\subseteq\bigcap\limits_{b\in
C(v)}s^R_{v,b}}}W_L(y_v,s_{v,C(v)})\cdot\left(\prod_{b\in
C(v)\setminus\{c\}}\rho^*_{b\rightarrow
v}(s^R_{v,b},s^R_{v,b})\right),
\end{equation}

\begin{equation}
\label{equ:sd_bp_rightmessage}\rho^*_{c\rightarrow
v}(s^R_{v,c},s^R_{v,c})=\sum_{{s^L_{V(c)\setminus\{v\},c}:}\atop{s^R_{v,c}={\tt
F}_c(s^L_{V(c)\setminus\{v\},c})}}W_R(s_{V(c),c})\cdot\left(\prod_{u\in
V(c)\setminus \{v\}}\lambda_{u\rightarrow c}(s^L_{u,c},{\tt
F}_c(s^R_{v,c}\times s^L_{V(c)\setminus\{u,v\},c}))\right).
\end{equation}

For the purpose of introducing a unified reduction from BP to SP, we
define the weighting function $W_L(y_v,s_{v,C(v)})$ as a conditional
function $W_L(y_v;s_{v,C(v)})$(???). We also define the weighting
function $W_R(s_{V(c),c})=1$.

\subsubsection{The reduction of SP from BP}

For each constraint $\Gamma_c$, we denote by $A_c(v)$ the set of
forced value of symbol variable $y_v$ in $\Gamma_c$. That is,
\[
A_c(v):= \{{\tt
F}_c(y_{V(c)\setminus\{v\}}):y_{V(c)\setminus\{v\}}\in
\chi^*_{V(c)\setminus\{v\}}\}.
\]

\begin{thm}
Given a CSP, for any $c\in C$ and $v\in V(c)$, let $a_{v,c}\in
A_c(v)$. If the following condition
\[
{\tt F}_c(a_{v,c}\times y_{V(c)\setminus\{u,v\}})\supseteq
\bigcap_{b\in C(u)\setminus\{c\}}a_{u,b}
\]
holds for any $u\in V(c)\setminus\{v\}$ and $y_{V(c)\setminus
\{u,v\}}\in \chi^*_{V(c)\setminus\{u,v\}}$, then the correspondence
of SD-BP message-passing rules
(\ref{equ:sd_bp_leftmessage})(\ref{equ:sd_bp_rightmessage}) and
PTP-$\gamma$ message-passing rules
(\ref{equ:ptpvtocGamma})(\ref{equ:ptpctov}) is
\[
\rho^*_{c\rightarrow v}(a_{v,c},a_{v,c})=\rho_{c\rightarrow v}
(a_{v,c}),
\]
where $(a_{v,c},a_{v,c})$ is in the support of $\rho^*_{c\rightarrow
v}$ and $a_{v,c}$ is in the support of $\rho_{c\rightarrow v}$.
\end{thm}

\begin{proof}
We can first merge SD-BP message-passing rules
(\ref{equ:sd_bp_leftmessage})(\ref{equ:sd_bp_rightmessage}) into
one, which is shown as follow.
\[
\rho^*_{c\rightarrow
v}(s^R_{v,c},s^R_{v,c})=\sum_{{s^L_{V(c)\setminus\{v\},c}:}\atop{s^R_{v,c}={\tt
F}_c}(s^L_{V(c)\setminus\{v\},c})}\prod_{u\in
V(c)\setminus\{v\}}\sum_{{s^R_{u,C(u)\setminus\{c\}}:}\atop{s^L_{u,c}\subseteq
Q}}W_L(s^L_{u,c},s_{u,C(u)})\cdot\left(\prod_{b\in C(u)\setminus
\{c\}}\rho^*_{b\rightarrow u}(s^R_{u,b},s^R_{u,b})\right),
\]
where $Q={\tt F}_c(s^R_{v,c}\times
s^L_{V(c)\setminus\{u,v\},c})\cap(\bigcap\limits_{b\in
C(u)\setminus\{c\}}s^R_{u,b})$.

Similarly, we can merge PTP-$\gamma$ message-passing rules
(\ref{equ:ptpvtocGamma})(\ref{equ:ptpctov})as follow.
\[
\rho_{c\rightarrow v}(t_{c\rightarrow
v})=\sum_{{t_{V(c)\setminus\{v\}\rightarrow
c}:}\atop{t_{c\rightarrow v}={\tt
F}_c}(t_{V(c)\setminus\{v\}\rightarrow c})}\prod_{v\in
V(c)\setminus\{v\}}\sum_{{t_{C(u)\setminus\{c\}\rightarrow
u}:}\atop{t_{u\rightarrow c}\subseteq \bigcap\limits_{b\in
C(u)\setminus\{c\}}t_{b\rightarrow u}}}\gamma(t_{u\rightarrow
c};t_{C(u)\setminus\{c\}\rightarrow u})\cdot\left(\prod_{b\in
C(u)\setminus\{c\}}\rho_{b\rightarrow u}(t_{b\rightarrow u})\right).
\]

We then have
\[
\rho^*_{c\rightarrow
v}(a_{v,c},a_{v,c})=\sum_{{s^L_{V(c)\setminus\{v\},c}:}\atop{a_{v,c}={\tt
F}_c}(s^L_{V(c)\setminus\{v\},c})}\prod_{u\in
V(c)\setminus\{v\}}\sum_{{s^R_{u,C(u)\setminus\{c\}}:}\atop{s^L_{u,c}\subseteq
Q}}W_L(s^L_{u,c},s_{u,C(u)})\cdot\left(\prod_{b\in C(u)\setminus
\{c\}}\rho^*_{b\rightarrow u}(s^R_{u,b},s^R_{u,b})\right),
\]
where $Q={\tt F}_c(a_{v,c}\times
s^L_{V(c)\setminus\{u,v\},c})\cap(\bigcap\limits_{b\in
C(u)\setminus\{c\}}s^R_{u,b})$, and
\[
\rho_{c\rightarrow
v}(a_{v,c})=\sum_{{t_{V(c)\setminus\{v\}\rightarrow
c}:}\atop{a_{v,c}={\tt F}_c}(t_{V(c)\setminus\{v\}\rightarrow
c})}\prod_{v\in
V(c)\setminus\{v\}}\sum_{{t_{C(u)\setminus\{c\}\rightarrow
u}:}\atop{t_{u\rightarrow c}\subseteq \bigcap\limits_{b\in
C(u)\setminus\{c\}}t_{b\rightarrow u}}}\gamma(t_{u\rightarrow
c};t_{C(u)\setminus\{c\}\rightarrow u})\cdot\left(\prod_{b\in
C(u)\setminus\{c\}}\rho_{b\rightarrow u}(t_{b\rightarrow u})\right).
\]

Since for any $c\in C$ and $\{u,v\}\subseteq V(c)$, we have ${\tt
F}_c(a_{v,c}\times
y_{V(c)\setminus\{u,v\}})\supseteq\bigcap\limits_{b\in
C(u)\setminus\{c\}}a_{u,b}$, then in SD-BP, we have

\begin{eqnarray*}
Q &=& {\tt F}_c(a_{v,c}\times
s^L_{V(c)\setminus\{u,v\},c})\cap(\bigcap\limits_{b\in
C(u)\setminus\{c\}}s^R_{u,b})\\
&=& \bigcap\limits_{b\in C(u)\setminus\{c\}}s^R_{u,b}.
\end{eqnarray*}

For each $c\in C$ and $v\in V(c)$, if we match
$s^L_{v,c}\leftrightarrow t_{v\rightarrow c}$ and
$s^R_{v,c}\leftrightarrow t_{c\rightarrow v}$, then we have
$\rho^*_{c\rightarrow v}(a_{v,c},a_{v,c})=\rho_{c\rightarrow
v}(a_{v,c})$. (There is one more step in this proof. It is to show
that, under that condition, the two weighting functions are the
same. This can be done after the definition of two functions are
given.)
\end{proof}


\subsection{$k$-SAT}

For any $v\in V$ in an instance of $k$-SAT problems, symbol variable
$y_v$ takes values from the extended alphabet
$\chi^*_v:=\{\emptyset,\{0\},\{1\},\{0,1\}\}$. For simplicity, we
introduce the following three symbols. We use symbol ${\tt F}$ to
denote the set $\{L_{v,c}\}$ and use symbol $\overline{\tt F}$ to
denote the set $\{\overline L_{v,c}\}$. We use symbol * to denote
the set $\{0,1\}$. Then the symbolic representation of the extended
alphabet is $\chi^*_v=\{\emptyset,{\tt F},\overline{\tt F}, *\}$.
For any $(x_v,\Gamma_c)$ on the factor graph representation, the
state variable $s_{v,c}$ takes values from the set
$\chi^*_v\times\chi^*_v$.

Given the local functions as shown in (\ref{equ:leftfunction}) and
(\ref{equ:rightfunction}), where the weighting functions are defined
as follows:

\[
 W_L(y_{v},s_{v,C(v)}) :=\left\{
\begin{array}{ll}
\omega_{*},&{\rm if} ~ n(s_{v, C(v)}^R; *)=|C(v)|\\
& ~{\rm and} ~ y_{v} = *  \\
\omega_{\tt u},&{\rm if} ~ n(s_{v, C(v)}^R; *)=|C(v)|
\\ & ~{\rm and} ~ y_{v} \neq *  \\
1, &{\rm otherwise},
\end{array}
\right.
\]
and
\[W_R(s_{V(c),c})=1,\]
we can get the global function shown in
($\ref{equ:globalfunction}$).

We say that a symbol-state configuration of $(y_V, s_{V, C})$ is
{\em valid} if it gives rise to non-zero value for function $F$. The
following lemma is easy to prove.

\begin{lem}
\label{lem:PMF} If $(y_V, s_{V, C})$ is a valid symbol-state
configuration under $F$, then
\begin{enumerate}
\item
for every state configuration $s_{v, c}$, it holds that
$s^R_{v,c}\neq \overline{\tt F}$, $s_{v, c}\neq \overline{\tt F}{\tt
F}$ and that $s_{v, c}\neq
*{\tt F}$, and
\item  $F(y_V, s_{V, C})=\omega_*^{n_*(y_V, s_{V, C})}
\cdot \omega_{\tt u}^{n_{\tt u}(y_V, s_{V, C})}$, where $n_*(y_V,
s_{V, C})$ and $n_{\tt u}(y_V, s_{V, C})$ are respectively the
cardinalities of set $\{v\in V: n(s_{v, C(v)}^R; *)=|C(v)|, y_v=*\}$
and set $\{v\in V: n(s_{v, C(v)}^R; *)=|C(v)|, y_v\neq *\}$.
\end{enumerate}
\end{lem}

\begin{proof}

\end{proof}

The first part of this lemma suggests that there are in fact only
four values that a state variable may take in valid symbol-state
configurations.

The second part of this lemma suggests that the PMF under this MRF
model is identical to that of \cite{SP:newlook}, since an equivalent
result is shown for the MRF in \cite{SP:newlook}. As such, the
reader is referred to \cite{SP:newlook} for a combinatorial
interpretation of the valid symbol configurations.

Now we consider applying the sum-product message-passing rule to the
Forney graphs, where we will use $\rho_{c\rightarrow v}$ to denote
the message passed from a right  function $f_c$ to a left function
$g_v$,  and use $\lambda_{v\rightarrow c}$ to denote the message
passed from left function $g_v$ to right function $f_c$. We note
that both $\rho_{c\rightarrow v}$  and $\lambda_{v\rightarrow c}$
are functions on the state space ${\cal L}\times {\cal R}$. The
first part of Lemma \ref{lem:PMF} implies that $\rho_{c\rightarrow
v}(\overline{\tt F}{\tt F})= \rho_{c\rightarrow v}(*{\tt F})=
\lambda_{v\rightarrow c}(\overline{\tt F}{\tt F})=
\lambda_{v\rightarrow c}(*{\tt F})=0$.  This makes each message a
quadruplet, the form of which is summarized in Lemma
\ref{lem:bp_mssg}.

\begin{lem}
\label{lem:bp_mssg} The sum-product message-passing rule applied on
the Forney graph defined earlier gives rise to:

\begin{equation*}\label{equ:rightMessage}
\begin{split}
  \rho_{c\rightarrow v} &
({\tt FF}) = \prod_{u\in V(c) \setminus \{v\}}\lambda_{u\rightarrow
c}
(\overline{\tt F}*),\\
 \rho_{c\rightarrow v} &
(\overline{\tt F}*) = \prod_{u\in V(c) \setminus \{v\}}
(\lambda_{u\rightarrow c}({\tt F}*)+\lambda_{u\rightarrow c}(**)
+\lambda_{u\rightarrow c}(\overline{\tt F}*) )\\
&+\sum_{u\in V(c)\setminus \{v\}} (\lambda_{u\rightarrow c}({\tt
FF})-\lambda_{u\rightarrow c}({\tt F}*) - \lambda_{u\rightarrow
c}(**))\times \prod_{w\in V(c)\setminus \{u, v\}}
\lambda_{w\rightarrow c}(\overline{\tt F}*)
-\prod_{u\in V(c)\setminus \{v\}} \lambda_{u\rightarrow c}(\overline{\tt F}*),\\
   \rho_{c\rightarrow v}&
({\tt F}*) = \prod_{u\in V(c) \setminus \{v\}}
(\lambda_{u\rightarrow c} ({\tt F}*)+\lambda_{u\rightarrow
c}(**)+\lambda_{u\rightarrow c}(\overline{\tt F}*)) -\prod_{u\in
V(c)\setminus \{v\}}\lambda_{u\rightarrow c}
(\overline{\tt F}*),\\
   \rho_{c\rightarrow v} & (**) = \prod_{u\in V(c) \setminus \{v\}}
(\lambda_{u\rightarrow c}({\tt F}*)+\lambda_{u\rightarrow
c}(**)+\lambda_{u\rightarrow c}(\overline{\tt F}*)) -\prod_{u\in
V(c)\setminus \{v\}} \lambda_{u\rightarrow c}(\overline{\tt F}*),
\end{split}
\end{equation*}

and

\begin{equation*}\label{equ:leftMessage}
\begin{split}
    \lambda_{v\rightarrow c} &
({\tt FF})= \prod_{b\in C_{c}^{\tt u}(v)}\rho_{b\rightarrow
v}(\overline{\tt F}*) \times \prod_{b\in C_{c}^{\tt
s}(v)}(\rho_{b\rightarrow v}({\tt FF})+
\rho_{b\rightarrow v}({\tt F}*)), \\
   \lambda_{v\rightarrow c} &
(\overline{\tt F}*)= \prod_{b\in C_{c}^{\tt s}(v)}\rho_{b\rightarrow
v} (\overline{\tt F}*) \times \left( \prod_{b\in C_{c}^{\tt
u}(v)}\left(\rho_{b\rightarrow v}({\tt F}*)+ \rho_{b\rightarrow
v}({\tt FF})\right)  \right. \left. -(1-\omega_{\tt u})\prod_{b\in
C_{c}^{\tt u}(v)}
\rho_{b\rightarrow v}({\tt F*})\right), \\
    \lambda_{v\rightarrow c} &
({\tt F}*)= \prod_{b\in C_{c}^{\tt u}(v)}\rho_{b\rightarrow
v}(\overline{\tt F}*) \times \left(\prod_{b\in C_{c}^{\tt
s}(v)}(\rho_{b\rightarrow v}({\tt F}*)+\rho_{b\rightarrow v}({\tt
FF}))\right.   \left. -(1-\omega_{\tt u})\prod_{b\in C_{c}^{\tt
s}(v)}\rho_{b\rightarrow v}({\tt F}*)
\right), \\
    \lambda_{v\rightarrow c}&
(**)= \omega_{*}\prod_{b\in C_{c}^{\tt u}(v)\cup C_{c}^{\tt
s}(v)}\rho_{b\rightarrow v}(**).
\end{split}
\end{equation*}
\end{lem}

\begin{thm}
\label{thm:sp_as_bp} Let $\omega_*$ equal $\gamma$, the parameter in
generalized SP. If the following conditions are imposed:1)
$\omega_{*}+\omega_{\tt u}=1$, 2)on every edge $(g_v, f_c)$ in the
Forney graph the BP messages are initialized such that
$\rho_{c\rightarrow v}({\tt F}*)=\rho_{c\rightarrow
v}(**)=\rho_{c\rightarrow v}(\overline{\tt F}*)$, and 3) normalize
$\rho_{c\rightarrow v}(\overline{\tt F}*)+\rho_{c\rightarrow v}({\tt
FF})=1$, then BP messages and SP messages are related by
\begin{equation*}
\begin{array}{lll}
\rho_{c\rightarrow v}({\tt FF}) & = &
\eta_{c\rightarrow v},\\
\lambda_{v\rightarrow c}(\overline{\tt F}*)& =& \Pi_{v\rightarrow
c}^{\tt u},
\end{array}
\end{equation*}

and
\[
\lambda_{v\rightarrow c}({\tt F}*)+ \lambda_{v\rightarrow c}(**)  =
\Pi_{v\rightarrow c}^{\tt s}+\Pi_{v\rightarrow c}^{*}.
\]
\end{thm}

That is, under the condition of this theorem, the SP($\gamma$)
message-passing rule is completely recovered.


\subsection{3-COL}


==> catchall.tex <==
\subsection{catch all}

\begin{enumerate}


\item ``intention-command''

\item use ``example'' enviroment whenever possible.

\item Check the use of ``followed by'' everywhere.

\item there is a latex-compiler warning saying that there are multiply defined labels. Must check, or check every reference of labels.


\item check consistency of heading fonts/style.


\item Theorem 1: the statement does not include summary message equivalence, although the proof contains it.



\item make uniform the term ``rectangle on U'' rather than ``rectangle supported by U''.

\item Make a remark on the NP-completeness of q-COL when introducing q-COL
(for which q?)





 
\item Is the condition for reduction of SDBP to PTP also sufficient for 
showing the summary messsage equivalence (between SDBP and PTP).






\item To decide whether in message-passing rule to use ``$=$'' or to 
use ``$:=$'' in defining messages. 

\item note somewhere that we are not concerned with decimation in this paper.

\item In some places, for consistency, we need to change $u$ to $v$ (or 
$v$ to $u$) such as in SP of 3COL versus PTP of 3COL.

\item mention $\rho({\bf i})$ for singleton token ${\bf i}$ is zero.

\item change of notations for SP message for 3COL: use $\eta_v$ rather 
than $\mu_v$ to refer to summary message; in the update rules, change $r$
to $i$, and change $p$ to either $j$ or $k$, to be consistent with the 
later notation in PTP.

\item Make extremely clear distinction between the term "variable" and
the term "varible vertex". Particularly, some places variable vertex $x_v$
does not mean "variable $x_v$".

\item ? to change notation $\eta^i$ to $\eta(i)$.











\item For token $a, b$, $a\subset b$ needs a definition, noting that they 
are ``assignments''.


\item make sure to use ``left('' and `` right)'' at where appropriate.

\end{enumerate}

 
{\bf [some analytical results need to be given for deterministic token
passing. Attempted below: For cycle-free FG, what is resulted upon convergence
if we are allowed to impose conditions on the initial tokens? If any, to what extent such results generalize to graph with cycles?
 
If the initial rectangle formed by the initial tokens is a singleton that is a
solution, then the resulting summary rectangle contains this solution.
If the initial rectangle is a bounding rectangle of all solutions, the resulting summary rectangle IS this bounding rectangle at convergence???? I guess not true. It could be bigger?
If the initial rectangle contains no solution, if each initial token
is valid (meaning, some solution projected on this coordinate is contained in
the token), and if the resulting token at each $v$ ``covers'' the initial
token at $v$, there?
 
 
This an additional unsatisfactory aspect of DTP. That is, the initial token is
not ``remembered'', they are over written as tokens are updated. Intuitively, this really bothers me. In away, there is no ``stablizing'' effect from the initial tokens that could force the resulting rectangle closely related to the
initial token in certain way. In a coding analogy, with tail-biting trellis,
the this corresponds to a pseudo codeword that starting from a state but does
not come back to the same state.]}
 

 
 




==> theorem1.tex <==
\begin{thm}
    Upon normalizing message $\lambda_{v\rightarrow c}$
to  $\lambda_{v\rightarrow c}^{\rm norm}$ in each PTP
    message-passing iteration such that
$\sum_{t}\lambda_{v\rightarrow
    c}^{\rm norm}(t)=1$, the correspondence between SP and PTP update rules
    on $3$-COL problems is
    \begin{eqnarray}
\label{equ:eqv_3col}
    &&\eta_{u\rightarrow v}^i=\lambda^{\rm norm}_{u\rightarrow\{u,v\}}(i)\\
        &&\eta_{u\rightarrow v}^*=\lambda^{\rm norm}_{u\rightarrow
        \{u,v\}}(ij)+\lambda^{\rm norm}_{u\rightarrow\{u,v\}}(ik)+\lambda^{\rm norm}_{u\rightarrow
        \{u,v\}}(jk)+\lambda^{\rm norm}_{u\rightarrow\{u,v\}}(ijk).
    \end{eqnarray}
\end{thm}

\begin{proof}
    First we will identify $c$ in the subscript of
    $\lambda_{u\rightarrow c}$ with constraint
    $\{u, v\}$ for which $v$ indexes the destination vertex in the subscript
    of  $\eta_{u\rightarrow v}$.
    Since the SP message $(\eta_{u \rightarrow v}^1, \eta_{u\rightarrow v}^2,
    \eta_{u\rightarrow v}^3, \eta_{u\rightarrow v}^*)$ is normalized, and
    so is the PTP message $\lambda_{u\rightarrow c}$ for any $c=\{u,v\}$, we only need to show the equivalence
    in Equation (\ref{equ:eqv_3col}) of the theorem.

    For any $c=\{u,v\}$, let $\alpha_{\{u,v\}}=\lambda^{\rm norm}_{u\rightarrow c}({\bf ij})+ \lambda^{\rm norm}_{u\rightarrow
    c}({\bf ik})+\lambda^{\rm norm}_{u\rightarrow c}({\bf jk})+\lambda^{\rm
    norm}_{u\rightarrow c}({\bf ijk})$. When applying PTP update equations (\ref{equ:ptp_3col_r_ij}) and
    (\ref{equ:ptp_3col_r_ijk}) to equations (\ref{equ:ptp_3col_l_i})
    to (\ref{equ:ptp_3col_l_ijk}), we have

    \begin{eqnarray}
    \lambda_{u\rightarrow c}({\bf i})& = &\prod_{b\in C(u)\setminus
    \{c\}}[1-\lambda^{\rm norm}_{V(b)\setminus\{u\}\rightarrow b}({\bf i})]-
    \prod_{b\in C(u)\setminus \{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}
    \rightarrow b}({\bf j})+\alpha_{\{V(b)\setminus\{u\},u\}}]]\\
    & &-\prod_{b\in C(u)\setminus \{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}
    \rightarrow b}({\bf k})+\alpha_{\{V(b)\setminus\{u\},u\}}]
    +\prod_{b\in C(u)\setminus \{c\}}
    \alpha_{\{V(b)\setminus\{u\},u\}}\nonumber\\
    \lambda_{u\rightarrow c}({\bf ij}) & = & \prod_{b\in
    C(u)\setminus\{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}\rightarrow
    b}({\bf k})+\alpha_{\{V(b)\setminus\{u\},u\}}]-\prod_{b\in
    C(u)\setminus\{c\}}\alpha_{\{V(b)\setminus\{u\},u\}}\\
    \lambda_{u\rightarrow c}({\bf ijk}) & = & \prod_{b\in
    C(u)\setminus\{c\}}\alpha_{\{V(b)\setminus\{u\},u\}}.
    \end{eqnarray}

    After normalization, we have
    \begin{eqnarray}
    \lambda^{\rm norm}_{u\rightarrow c}({\bf i})& = &\frac{1}{\beta}\cdot\left(\prod_{b\in C(u)\setminus
    \{c\}}[1-\lambda^{\rm norm}_{V(b)\setminus\{u\}\rightarrow b}({\bf i})]-
    \prod_{b\in C(u)\setminus \{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}
    \rightarrow b}({\bf j})+\alpha_{\{V(b)\setminus\{u\},u\}}]\right.\nonumber\\
    & &\left. -\prod_{b\in C(u)\setminus \{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}
    \rightarrow b}({\bf k})+\alpha_{\{V(b)\setminus\{u\},u\}}]
    +\prod_{b\in C(u)\setminus \{c\}}
    \alpha_{\{V(b)\setminus\{u\},u\}}\right)\\
    \lambda^{\rm norm}_{u\rightarrow c}({\bf ij}) & = &\frac{1}{\beta}\cdot\left(\prod_{b\in
    C(u)\setminus\{c\}}[\lambda^{\rm norm}_{V(b)\setminus\{u\}\rightarrow
    b}({\bf k})+\alpha_{\{V(b)\setminus\{u\},u\}}]-\prod_{b\in
    C(u)\setminus\{c\}}\alpha_{\{V(b)\setminus\{u\},u\}}\right)\\
    \lambda^{\rm norm}_{u\rightarrow c}({\bf ijk}) & = &\frac{1}{\beta}\cdot\prod_{b\in
    C(u)\setminus\{c\}}\alpha_{\{V(b)\setminus\{u\},u\}},
    \end{eqnarray}
    where $\beta=\sum_{i=1,2,3}\prod_{b\in C(u)\setminus\{c\}}[1-\lambda^{\rm norm}_{V(b)
    \setminus\{u\}\rightarrow b}({\bf i)}]-\sum_{i=1,2,3}
    \prod_{b\in C(u)\setminus\{c\}}[\lambda^{\rm
    norm}_{V(b)\setminus\{u\}\rightarrow b}({\bf
    i})+\alpha_{\{V(b)\setminus\{u\},u\}}]+\prod_{b\in
    C(u)\setminus\{c\}}\alpha_{\{V(b)\setminus\{u\},u\}}$.

    For any $c=\{u,v\}$, it is clear that $\lambda^{\rm norm}_{u\rightarrow c}({\bf i})
    =\eta^{i}_{u\rightarrow v}$ and $\alpha_{\{u,v\}}=\eta^*_{u\rightarrow
    v}$.
    \end{proof}

